Group Fairness in Bandit Arm Selection

We propose a novel formulation of group fairness with biased feedback in the contextual multi-armed bandit (CMAB) setting. In the CMAB setting, a sequential decision maker must, at each time step, choose an arm to pull from a finite set of arms after observing some context for each of the potential arm pulls. In our model, arms are partitioned into two or more sensitive groups based on some protected feature(s) (e.g., age, race, or socio-economic status). Initial rewards received from pulling an arm may be distorted due to some unknown societal or measurement bias. We assume that in reality these groups are equal despite the biased feedback received by the agent. To alleviate this, we learn a societal bias term which can be used to both find the source of bias and to potentially fix the problem outside of the algorithm. We provide a novel algorithm that can accommodate this notion of fairness for an arbitrary number of groups, and provide a theoretical bound on the regret for our algorithm. We validate our algorithm using synthetic data and two real-world datasets for intervention settings wherein we want to allocate resources fairly across groups.

==> naive.tex <==
Much of the research on fairness in machine learning focuses on fairness in classification~\cite{Dwork12:Fairness}. One popular definition of group fairness in classification is the Rawlsian notion of demographic parity \cite{Rawls71a}.  Formally, given a protected demographic group $A$, we want:
{\small
 \begin{equation}
     \Pr(\hat{Y}=1 | A=0) = \Pr(\hat{Y}=1 | A=1),
 \end{equation}
 }
where the probability of assigning a classification label $\hat{Y}=1$ does not change based on the sensitive attribute class $A$. Demographic parity is important when ground truth classes $Y$ are extremely noisy for sensitive groups due to some societal or measurement bias. Assume that we have a classifier that predicts whether an individual should receive a loan where our sensitive attribute $A$ is binary gender. Demographic parity states that the probability of getting a loan should be the same for males ($A= 0$) and females ($A=1$).

In converting this definition of demographic parity to the the multi-armed bandit setting, we alter the definition to be that the probability of pulling an arm $a$ does not change based on group membership $P_j$: 
{\small
\begin{equation}
    \Pr(\textit{pull } a | a\in P_0) = \Pr(\textit{pull } a | a\in P_1).
\end{equation}
}

% Alternatively, we can use a definition of proportional parity to be the probability of pulling an arm $a$ where $a\in P_j$ should be proportional to the size of the group $P_j$:
% \begin{equation}
%     \Pr(\textit{pull } a | a\in P_j) = \frac{|P_j|}{n}.
% \end{equation}

Continuing our running example, assume we are a loan agency. The loan agency receives 4 applications at every timestep $t$: an applicant from a young female, an applicant from a young male, an applicant from a older female, an applicant from an older male; we must choose one application to grant at each timestep. After granting a loan the loan agency receives a down payment on that loan as reward. This reward is then used to update the estimates of whether or not a ``good'' loan application was received for the pulled arm. Assume that the loan agency wants to act fairly using the binary sensitive attribute of gender.  Then, the probability that the loan agency chooses a female applicant at timestep $t$ should be the same as the probability of choosing a male applicant.



\subsection{A Motivating Example: Linear Regret}

\begin{algorithm}
\caption{\NaiveGroupFair{}}\label{alg:naive}
\begin{algorithmic}[1]
\REQUIRE $\delta$, $P_1$, $P_2$
\FOR{$t=1\ldots T$}
\STATE $P \gets$ Randomly choose group $P_1$ or $P_2$.
\STATE Pull arm in $P$ based on \textsc{TopInterval}
\ENDFOR
%
\end{algorithmic}
\end{algorithm}

A naive algorithm to enforce this definition of fairness is defined in Algorithm~\ref{alg:naive}. We first pick from the groups uniformly at random, and then apply a regular CMAB algorithm like \textsc{TopInterval}\footnote{\textsc{TopInterval} is a variant of the contextual bandit LinUCB by \citet{Auer:02:UCB}.} or \textsc{ContextualThompsonSampling} \cite{Agrawal:13:ThompsonSampling} to choose which arm to pull within the group. Using our running example, \NaiveGroupFair{} would randomly pick between male or female, and then choose the best applicant between the younger and older pair.

Assume that \NaiveGroupFair{} randomly chooses the male group during the first timestep and at this timestep the two best applicants are in the female group. Assume that by chance, this worst-case scenario happens at every timestep $t$. We can extend this argument to any constant number of groups, hence this shows that we have a linear regret for Algorithm~\ref{alg:naive}.

% \nick{Perhaps revise the above last sentece to be: We can extend this argument to any constant number of groups -- hence this shows ...}

% \nick{We said: To clarify, if you force an algorithm to spread arm pulls evenly across 2 groups, and by chance one of those groups contains all the objects you want, then you'll end up with at least $1/2 * (\text{difference between the best arm in the worse group and the arms in the other group}) * T$ = $1/2 * (\text{positive constant}) * T$ = $(\text{positive constant}) * T$ = $O(T)$ regret.  This argument extends to any constant number of groups. }





% Let us assume we have two arms $a$ and $b$ and that $a \in P_1$ while $b \in P_2$. Let's assume that algorithm~\ref{alg:naive} randomly picks $P_1$. We therefore pull arm $a$. Let's assume that was the incorrect choice and arm $b$ had a higher reward. Theoretically this can happen for every round $t$ in $T$. Therefore we have linear regret for Algorithm~\ref{alg:naive}. \cs{Expand using running example}
% \begin{theorem}\label{thm:linear_bound}
% For two groups $P_1$ and $P_2$ \NaiveGroupFair{} has regret
% \begin{equation}
%     R(T)=O\left(T\right)
% \end{equation}
% \end{theorem}

We could, then, just focus on inner group regret,
{\small
\begin{equation*}
    R(t) = f(x_{i^*,t}) - f(x_{a,t}) \quad\text{ where } i,a\in P_j,
\end{equation*}
}
instead of overall regret (Equation~\ref{eq:orig_regret}).
In other words, we could focus on the regret of choosing between the younger and older applicant for both genders. This separates the arms into two CMAB problems. This is unsatisfying as it ignores and removes the interaction and differences between groups. We therefore suggest that a new definition of regret that includes a concept of societal bias is needed in this case.

